Parametric error bounds for convex approximations of two-stage mixed-integer recourse models with a random second-stage cost vector

We consider two-stage recourse models in which the second-stage problem has integer decision variables and uncertainty in the second-stage cost vector, technology matrix, and the right-hand side vector. Such mixed-integer recourse models are typically non-convex and thus hard to solve. There exist convex approximations of these models with accompanying error bounds. However, it is unclear how these error bounds depend on the distributions of the second-stage cost vector $q$. In fact, the only error bound that is known hinges on the assumption that $q$ has a finite support. In this paper, we derive parametric error bounds whose dependence on the distribution of $q$ is explicit and that hold for any distribution of $q$, provided it has a finite expected $\ell_1$-norm. We find that the error bounds scale linearly in the expected value of the $\ell_1$-norm of $q$.

==> Figures/Capacity2Nodes.tex <==
\begin{tikzpicture}[scale=0.6]
    % Draw axes
    \coordinate (o) at (0,0);
    \coordinate (xmax) at (4,0);
    \coordinate (ymax) at (0,8);
    \draw[->] (o) -- (xmax);
    \node[right=0mm of xmax]{$f$};
    \draw[->] (o) -- (ymax);
    \node[above=0mm of ymax]{$\pi$};
    
    % Draw residual demand curve
    \draw[domain=0:4,smooth,variable=\x,blue] plot ({\x},{7.33-0.67*\x});
    \coordinate (p1star) at (0,7.33);
    \node[left=0mm of p1star]{$\pi_1^*$};
    
    % Draw residual supply curve
    \draw[domain=0:4,smooth,variable=\x,red] plot ({\x},{0.67*\x+4});
    \coordinate (p2star) at (0,4);
    \node[left=0mm of p2star]{$\pi_2^*$};
    
    % Draw optimal capacity
    \coordinate (kopt) at (1.53,0);
    \draw[dashed] (kopt) -- (1.53,6.32);
    \node[below=0mm of kopt]{$x^\prime$};
    
    % Draw equilibrium prices
    \coordinate (p1) at (0,6.32);
    \coordinate (p2) at (0,5.02);
    \coordinate (opt1) at (1.53,6.32);
    \coordinate (opt2) at (1.53,5.02);
    \coordinate (pnew) at (0,5.67);
    \coordinate (optnew) at (2.5, 5.67);
    \draw[dashed] (p1) -- (opt1);
    \node[left=0mm of p1]{$\pi_1'$};
    \fill[black] (opt1) circle (3pt);
    \draw[dashed] (p2) -- (opt2);
    \node[left=0mm of p2]{$\pi_2'$};
    \fill[black] (opt2) circle (3pt);
    \draw[dashed] (pnew) -- (optnew);
    \node[left=1mm of pnew]{$\bar{\pi}$};
    
    % Draw surplus change region 1
    \fill[green,opacity=0.2] plot coordinates {(0,7.33)(opt1)(p1)};
    
    % Draw surplus change region 2
    \fill[magenta,opacity=0.2] plot coordinates {(0,4)(opt2)(p2)};
    
    % Draw congestion rent
    \fill[brown,opacity=0.2] plot coordinates {(p1)(opt1)(opt2)(p2)};
    
    % Draw maximum capacity expansion
    \coordinate (opt) at (2.5,8);
    \coordinate (kmax) at (2.5,0);
    \draw[dashed] (kmax) -- (opt);
    \node[below=0mm of kmax]{$\bar{f}$};
\end{tikzpicture}

==> Figures/Network2Nodes.tex <==
\begin{tikzpicture}[scale=0.5]
    \coordinate (n1) at (0,0);
    \coordinate (n2) at (2,0);
    \draw[dashed] (n1) -- (n2);
    \fill[black] (n1) circle (3pt);
    \fill[black] (n2) circle (3pt);
    \node[above=1mm of n1] {1};
    \node[above=1mm of n2] {2};
\end{tikzpicture}

==> Figures/Network3NodesRadial.tex <==
\begin{tikzpicture}[scale=0.5]
    \coordinate (n1) at (0,0);
    \coordinate (n2) at (2,0);
    \coordinate (n3) at (4,0);
    \draw (n1) -- (n2);
    \draw[dashed] (n2) -- (n3);
    \fill[black] (n1) circle (3pt);
    \fill[black] (n2) circle (3pt);
    \fill[black] (n3) circle (3pt);
    \node[above=1mm of n1] {1};
    \node[above=1mm of n2] {2};
    \node[above=1mm of n3] {3};
\end{tikzpicture}

==> Figures/Surplus2Nodes.tex <==
\begin{tikzpicture}[scale=0.6]
    % Draw axes
    \draw [<->] (0,11) node (yaxis) [above] {$\pi_1$} |- (5,0) node (xaxis) [below] {$q_1$};
    % Draw demand curve
    \draw[domain=0:5,smooth,variable=\x,blue] plot ({\x},{10-\x});
    % Draw supply curve
    \draw[domain=0:4,smooth,variable=\x,red] plot ({\x},{2+2*\x});
    % Draw uncapacitated optimum
    \coordinate (uncap) at (2.67,7.33);
    \fill[black] (uncap) circle (3pt);
    \draw[dashed] (yaxis |- uncap) node[left] {$\pi_1^*$} -| (xaxis -| uncap) node[below] {$q_1^*$};
    % Draw capacitated optimum
    \coordinate (capdem) at (3.68,6.32);
    \coordinate (capsup) at (2.16,6.32);
    \coordinate (p2) at (3.68,5.02);
    \fill[black] (capdem) circle (3pt);
    \draw[dashed] (yaxis |- capsup) node[left] {$\pi_1^\prime$} -| (xaxis -| capdem) node[below] {$d_1^\prime$};
    \fill[black] (capsup) circle (3pt);
    \draw[dashed] (capsup |- capdem) node[left] {} -| (xaxis -| capsup) node[below] {$s_1^\prime$};
    % Draw consumer surplus
    \fill[green,opacity=0.2] plot coordinates {(0,10)(0,6.32)(3.68,6.32)};
    % Draw producer surplus
    \fill[magenta,opacity=0.2] plot coordinates {(0,6.32)(2.16,6.32)(0,2)};
    % Draw congestion rent
    \fill[brown,opacity=0.2] plot coordinates {(2.16,6.32)(3.68,6.32)(3.68,5.02)(2.16,5.02)};
    \draw[dashed] (0,5.02) node [left] {$\pi_2^\prime$} -- (3.68,5.02);
\end{tikzpicture}
\quad
\begin{tikzpicture}[scale=0.6]
    % Draw axes
    \draw [<->] (0,11) node (yaxis) [above] {$\pi_2$} |- (6,0) node (xaxis) [below] {$q_2$};
    % Draw demand curve
    \draw[domain=0:5,smooth,variable=\x,blue] plot ({\x},{10-2*\x});
    % Draw supply curve
    \draw[domain=0:6,smooth,variable=\x,red] plot({\x},{1+\x});
    % Draw uncapacitated optimum
    \coordinate (uncap) at (3,4);
    \fill[black] (uncap) circle (3pt);
    \draw[dashed] (yaxis |- uncap) node[left] {$\pi_2^*$} -| (xaxis -| uncap) node[below] {$q_2^*$};
    % Draw capacitated optimum
    \coordinate (capdem) at (2.49,5.02);
    \coordinate (capsup) at (4.02,5.02);
    \fill[black] (capdem) circle (3pt);
    \draw[dashed] (yaxis |- capdem) node[left] {$\pi_2^\prime$} -| (xaxis -| capdem) node[below] {$d_2^\prime$};
    \fill[black] (capsup) circle (3pt);
    \draw[dashed] (capdem |- capsup) node[left] {} -| (xaxis -| capsup) node[below] {$s_2^\prime$};
    % Draw consumer surplus
    \fill[green,opacity=0.2] plot coordinates {(0,10)(0,5.02)(2.49,5.02)};
    % Draw producer surplus
    \fill[magenta,opacity=0.2] plot coordinates {(0,5.02)(4.02,5.02)(0,1)};
\end{tikzpicture}

==> Figures/Surplus3Nodes.tex <==
\begin{tikzpicture}[scale=0.6]
    % Draw axes
    \draw [<->] (0,8) node (yaxis) [above] {$\pi$} |- (8,0) node (xaxis) [below] {$f$};
    % Draw excess demand curve
    \draw[domain=0:6,smooth,variable=\x,blue] plot ({\x},{6 - \x});
    \node at (6,1.5) {\textcolor{blue}{$I_2(\pi)$}};
    % Draw excess supply curve
    \draw[domain=0:6,smooth,variable=\x,red] plot({\x},{\x});
    \node at (6,4.5) {\textcolor{red}{$E_1(\pi)$}};
    % Draw old optimum
    \coordinate (opt) at (3,3);
    \fill[black] (opt) circle (3pt);
    \draw[dashed] (yaxis |- opt) node[left] {$\pi^{\text{old}}$} -| (xaxis -| opt) node[below] {$f^{\text{old}}$};
    % Draw consumer surplus
    \fill[green,opacity=0.2] plot coordinates {(0,6)(0,3)(3,3)};
    % Draw producer surplus
    \fill[magenta,opacity=0.2] plot coordinates {(0,0)(0,3)(3,3)};
\end{tikzpicture}
\quad
\begin{tikzpicture}[scale=0.6]
    % Draw axes
    \draw [<->] (0,8) node (yaxis) [above] {$\pi$} |- (8,0) node (xaxis) [below] {$f$};
    % Draw excess demand curve
    \draw[domain=0:6,smooth,variable=\x,blue] plot ({\x},{6 - 0.5*\x});
    \node at (6.5,2.5) {\textcolor{blue}{$I_{2,3}(\pi)$}};
    % Draw excess supply curve
    \draw[domain=0:6,smooth,variable=\x,red] plot({\x},{\x});
    \node at (6.5,5) {\textcolor{red}{$E_1(\pi)$}};
    % Draw new optimum
    \coordinate (optnew) at (4,4);
    \fill[black] (optnew) circle (3pt);
    \draw[dashed] (yaxis |- optnew) node[left] {$\pi^{\text{new}}$} -| (xaxis -| optnew) node[below] {$f^{\text{new}}$};
    % Draw consumer surplus
    \fill[green,opacity=0.2] plot coordinates {(0,6)(0,4)(4,4)};
    % Draw producer surplus
    \fill[magenta,opacity=0.2] plot coordinates {(0,0)(0,4)(4,4)};
\end{tikzpicture}
